Revisiting Ranking for Online Bipartite Matching with Random Arrivals: the Primal-Dual Analysis

We revisit the celebrated Ranking algorithm by Karp, Vazirani, and Vazirani (STOC 1990) for online bipartite matching under the random arrival model, that is shown to be $0.696$-competitive for unweighted graphs by Mahdian and Yan (STOC 2011) and $0.662$-competitive for vertex-weighted graphs by Jin and Williamson (WINE 2021). In this work, we explore the limitation of the primal-dual analysis of Ranking and aim to bridge the gap between unweighted and vertex-weighted graphs. We show that the competitive ratio of Ranking is between $0.686$ and $0.703$, under our current knowledge of Ranking and the framework of primal-dual analysis. This confirms a conjecture by Huang, Tang, Wu, and Zhang (TALG 2019), stating that the primal-dual analysis could lead to a competitive ratio that is very close to $0.696$. Our analysis involves proper discretizations of a variational problem and uses LP solver to pin down the numerical number. As a bonus of our discretization approach, our competitive analysis of Ranking applies to a more relaxed random arrival model. E.g., we show that even when each online vertex arrives independently at an early or late stage, the Ranking algorithm is at least $0.665$-competitive, beating the $1-1/e \approx 0.632$ competitive ratio under the adversarial arrival model.

==> certification.tex <==
\section{Lower Bound: Certification}

Lower Bound: certification
\begin{itemize}
\item Enumerating all ${2n \choose n}$ possible $\beta_n$.
\item (Explaination) Point-wise minimization for $\alpha_n$
\end{itemize}

==> heuristic.tex <==
\section{Upper Bound: Heuristic}
\begin{itemize}
\item Size of the optimization $\check{\Gamma},\hat{\Gamma}$:
\begin{itemize}
\item number of variables: $n^2+1$
\item monotone constraints: ...
\item $f(x,y) + f(y,x) \le 1, \forall x,y \in \grid$
\item $C(\alpha_n,\beta_n)$: roughly $n^n \cdot {2n\choose n}$ number of constraints
\end{itemize}
\item Heuristic for solving $\check{\Gamma},\hat{\Gamma}$:
\begin{itemize}
\item number of variables: $n^2+1$
\item monotone constraints: ...
\item $f(x,y) + f(y,x) \le 1, \forall x,y \in \grid$
\item Restrict ourselves to monotone $\alpha_n$, still $\left({2n \choose n}\right)^2$ number of constraints
\item Definition: Local perturbation to $\alpha_n$, figures
\item Iterative optimization:
\item Let $f^*, \Gamma^*$ be the optimal solution from the last iteration.
\item Let $S$ be the set of binding pairs $(\alpha_n, \beta_n)$ from the last iteration.
\item Let $T = S$.
\item Check all local perturbations and if $\Gamma(f^*,\alpha',\beta) < \Gamma^*$, add $(\alpha',\beta)$ to $T$.
\item Solve optimization w.r.t. $T$.
\end{itemize}
\item n=20: $10^{22}$ constraints. Need Figure: (ratio, iteration), (size of binding constraints, iteration)
\item Figure: (n,ratio)
\end{itemize}
